On the Selection of Random Field Evaluation Points in the p-MLQMC Method

Engineering problems are often characterized by significant uncertainty in their material parameters. A typical example coming from geotechnical engineering is the slope stability problem where the soil's cohesion is modeled as a random field. An efficient manner to account for this uncertainty is the novel sampling method called p-refined Multilevel Quasi-Monte Carlo (p-MLQMC). The p-MLQMC method uses a hierarchy of p-refined Finite Element meshes combined with a deterministic Quasi-Monte Carlo sampling rule. This combination yields a significant computational cost reduction with respect to classic Multilevel Monte Carlo. However, in previous work, not enough consideration was given how to incorporate the uncertainty, modeled as a random field, in the Finite Element model with the p-MLQMC method. In the present work we investigate how this can be adequately achieved by means of the integration point method. We therefore investigate how the evaluation points of the random field are to be selected in order to obtain a variance reduction over the levels. We consider three different approaches. These approaches will be benchmarked on a slope stability problem in terms of computational runtime. We find that for a given tolerance the Local Nested Approach yields a speedup up to a factor five with respect to the Non-Nested approach.

==> Rates/Legend_times.tex <==

\begin{tikzpicture}
\begin{axis}[%
    hide axis,
    xmin=10,
    xmax=50,
    ymin=0,
    ymax=0.4,
    legend style={draw=white!15!black,legend cell align=left,legend columns=-1},
    every axis plot/.append style={thick}
    ]
    \addlegendimage{black,mark=square*}
    \addlegendentry{$T_{\ell}$ h-ML(Q)MC};

    
    \addlegendimage{black,dotted, mark=square*,line width={1.5pt}}
    \addlegendentry{$T_{\ell}$ p-ML(Q)MC};
    \end{axis}
\end{tikzpicture}


==> Runtime/run_time_case.tex <==
%\RequirePackage{luatex85}
%\documentclass[tikz]{standalone}
%% Default preamble
%\usepackage{pgfplots}
%\pgfplotsset{compat=newest}
%\usepgfplotslibrary{groupplots}
%\usepgfplotslibrary{polar}
%\usepgfplotslibrary{statistics}
%\usepgfplotslibrary{dateplot}
%% Custom preamble from global variable:
%\usepackage{amsfonts}
\newcommand{\littletriangle}[4]
{
    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xBrel}

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax]
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax]
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax]
        \pgfmathsetmacro{\lnyC}{\lnyA+1.1*#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
        
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        \draw[black]   (A)--node[pos=0.9,yshift=1ex,xshift=0.5ex] {\small #4}
                    (B)--
                    (C)-- 
                    cycle;
    }
}

%\newcommand{\drawsquare}[3]{\draw[thick,black,fill=#3] (#1,#2)--(#1,#2+1)--(#1+1,#2+1)--(#1+1,#2)--cycle;}


%\begin{document}
\begin{tikzpicture}
\begin{axis}[ticklabel style={{font=\Large}}, major tick length={2pt}, every tick/.style={{black, line cap=round}}, axis on top, legend style={{draw=none, font=\Large, at={(0.03,0.03)}, anchor=south west,ymin=10^3,ymax=500000,xmin=10^-6,xmax=0.2*10^-2, fill=none, legend cell align=left}}, xmode={log}, ymode={log}, legend style={{draw=none, font=\small, at={(0.97,0.97)}, anchor=north east, fill=none, legend cell align=left}}, xlabel={\Large RMSE $\varepsilon$ [/]}, ylabel={\Large Total Runtime [sec] },legend style={font=\scriptsize},every axis plot/.append style={thick}]


        
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%NON NESTED

        
        \addplot[mark={*}, mark size={2.5pt}, line cap={round}, mark options={solid}, color={rgb,255:red,255;green,89;blue,77}]
        table[row sep={\\}]
        {
            \\
%            0.0028780652145494676  1392.553488366  \\
%            0.002213896318884206  1392.562828273  \\
%            0.0017029971683724659  1392.571557067  \\
%            0.0013099978218249738  1392.580305745  \\
            0.0010076906321730566  1392.589788555  \\
            0.0007751466401331204  1499.116165098  \\
            0.0005962666462562465  2229.685932418  \\
            0.00045866665096634343  3798.383058392  \\
            0.0003528205007433411  4666.87521623  \\
            0.00027140038518718546  6998.41890013  \\
            0.00020876952706706575  9662.338709519001  \\
            0.00016059194389774287  11170.370453761001  \\
            0.00012353226453672527  12445.191698279  \\
            9.502481887440405e-5  17253.512574052  \\
            7.309601451877234e-5  45844.521395515  \\
            5.6227703475978725e-5  98068.547500047  \\
            4.3252079596906715e-5  113784.71808462  \\
            3.3270830459159006e-5  158643.250524008  \\
            2.559294650704539e-5  179198.12480239902  \\
        }
        ;
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%GLOBAL NESTED

        \addplot[mark={triangle*}, mark size={2.5pt}, line cap={round}, mark options={solid}, color={rgb,255:red,255;green,122;blue,40}]
        table[row sep={\\}]
        {
            \\
%                        0.0028780652145494676  1432.111537889  \\
%            0.002213896318884206  1432.1198854689999  \\
%            0.0017029971683724659  1432.162074638  \\
%            0.0013099978218249738  1432.170760256  \\
            0.0010076906321730566  1432.17983979  \\
            0.0007751466401331204  1432.187937653  \\
            0.0005962666462562465  1534.1275505410001  \\
            0.00045866665096634343  1534.135879909  \\
            0.0003528205007433411  1738.8092644160001  \\
            0.00027140038518718546  2101.262456377  \\
            0.00020876952706706575  2785.984834058  \\
            0.00016059194389774287  3555.556501421  \\
            0.00012353226453672527  5740.9016060270005  \\
            9.502481887440405e-5  16470.165632526  \\
            7.309601451877234e-5  30199.111752041  \\
            5.6227703475978725e-5  30199.134572595  \\
            4.3252079596906715e-5  46027.701845376  \\
            3.3270830459159006e-5  62711.228021029005  \\
            2.559294650704539e-5  78172.790794912  \\
            1.9686881928496454e-5  174115.54016797198  \\
            1.5143755329612655e-5  201535.94317844798  \\
            1.1649042561240503e-5  359078.771626591  \\
            8.960801970185002e-6  386731.619150483  \\
            6.892924592450002e-6  409886.1111666  \\
        }
        ;
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%LOCAL NESTED




        \addplot[mark={star}, mark size={2.5pt}, line cap={round}, mark options={solid}, color={rgb,255:red,0;green,179;blue,89}]
        table[row sep={\\}]
        {
            \\
%            0.0028780652145494676  1394.635561854  \\
%            0.002213896318884206  1394.6457996079998  \\
%            0.0017029971683724659  1394.655382903  \\
%            0.0013099978218249738  1394.664975403  \\
            0.0010076906321730566  1394.674117474  \\
            0.0007751466401331204  1513.76868102  \\
            0.0005962666462562465  1615.270915998  \\
            0.00045866665096634343  1615.28072223  \\
            0.0003528205007433411  1826.729219825  \\
            0.00027140038518718546  1940.08149537  \\
            0.00020876952706706575  2216.705233958  \\
            0.00016059194389774287  2861.420945565  \\
            0.00012353226453672527  3906.010863614  \\
            9.502481887440405e-5  7964.152523104  \\
            7.309601451877234e-5  14837.940291211999  \\
            5.6227703475978725e-5  22132.376330648  \\
            4.3252079596906715e-5  24863.829800476  \\
            3.3270830459159006e-5  39890.349014228  \\
            2.559294650704539e-5  61909.941822295  \\
            1.9686881928496454e-5  108306.554055671  \\
            1.5143755329612655e-5  129677.928817426  \\
            1.1649042561240503e-5  193327.189082957  \\
            8.960801970185002e-6  252256.644228723  \\
            6.892924592450002e-6  350587.045230027  \\
            5.302249686500001e-6  403071.36628732097  \\
        }
        ;
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5         


% \addplot[dashed,mark={none}, color={black}]
%        table[row sep={\\}]
%        {
%            \\
%            3.e-6  542223  \\
%            0.0006  542223  \\
%        } 
%        ;   

            \addplot[dashed,mark={none}, color={black}]
        table[row sep={\\}]
        {
            \\
            3.e-6  302400  \\
            0.0006  302400  \\
        } 
        ; 
        
                    \addplot[dashed,mark={none}, color={black}]
        table[row sep={\\}]
        {
            \\
            3.e-6  172800  \\
            0.0006  172800  \\
        } 
        ; 


            \addplot[dashed,mark={none}, color={black}]
        table[row sep={\\}]
        {
            \\
            3.e-6  86400  \\
            0.0006  86400  \\
        } 
        ;   
        
        
                     \addplot[dashed,mark={none}, color={black}]
        table[row sep={\\}]
        {
            \\
            3.e-6  43200  \\
            0.0006  43200  \\
        } 
        ; 
        
                     \addplot[dashed,mark={none}, color={black}]
        table[row sep={\\}]
        {
            \\
            3.e-6  21600  \\
            0.0006  21600  \\
        } 
        ; 
        
        
%                                     \addplot[dashed,mark={none}, color={black}]
%        table[row sep={\\}]
%        {
%            \\
%            5.e-5  18000  \\
%            0.0007  18000  \\
%        } 
%        ; 
        
%                                             \addplot[dashed,mark={none}, color={black}]
%        table[row sep={\\}]
%        {
%            \\
%            5.e-5  14400  \\
%            0.0007  14400  \\
%        } 
%        ; 
        
                             \addplot[dashed,mark={none}, color={black}]
        table[row sep={\\}]
        {
            \\
            3.e-6  10800  \\
            0.0006  10800  \\
        } 
        ; 
        
                            \addplot[dashed,mark={none}, color={black}]
        table[row sep={\\}]
        {
            \\
            3.e-6  7200  \\
            0.0006  7200  \\
        } 
        ; 
        
                                    \addplot[dashed,mark={none}, color={black}]
        table[row sep={\\}]
        {
            \\
            3.e-6  3600  \\
            0.0006  3600  \\
        } 
        ; 


%          \node[black] at (axis cs:0.0009,542223){\normalsize{156 h}};
          \node[black] at (axis cs:0.0009,302400){\normalsize{84 h}};
%          \node[black] at (axis cs:0.0009,259200){\normalsize{72 h}};


%          \node[black] at (axis cs:0.0009,216000){\normalsize{60 h}};

          \node[black] at (axis cs:0.0009,172800){\normalsize{48 h}};

%          \node[black] at (axis cs:0.0009,129600){\normalsize{36 h}};

          \node[black] at (axis cs:0.0009,86400){\normalsize{24 h}};
          \node[black] at (axis cs:0.0009,43200){\normalsize{12 h}};
         \node[black] at (axis cs:0.0009,21600){\normalsize{6 h}};
 
 
 %                 \node[black] at (axis cs:0.0009,18000){\large{5 h}};
  %                \node[black] at (axis cs:0.0009,14400){\large{4 h}};

                  \node[black] at (axis cs:0.0009,10800){\normalsize{3 h}};

                   \node[black] at (axis cs:0.0009,7200){\normalsize{2 h}};

%          \node[black] at (axis cs:0.00020,7200){\normalsize{2 h}};
          \node[black] at (axis cs:0.0009,3600){\normalsize{1 h}};
%          \node[black] at (axis cs:0.00023,900){\normalsize{15 min}};


 %  \littletriangle{0.15}{0.1}{0.45}{2};
  %  \littletriangle{0.15}{0.1}{0.27}{1};
\end{axis}
\node at (3.5,6.5) {\Large ---Absolute Runtime---};

\end{tikzpicture}
%\end{document}


==> Runtime/run_time_case_Normalized.tex <==
%\RequirePackage{luatex85}
%\documentclass[tikz]{standalone}
%% Default preamble
%\usepackage{pgfplots}
%\pgfplotsset{compat=newest}
%\usepgfplotslibrary{groupplots}
%\usepgfplotslibrary{polar}
%\usepgfplotslibrary{statistics}
%\usepgfplotslibrary{dateplot}
%% Custom preamble from global variable:
%\usepackage{amsfonts}
\newcommand{\littletriangle}[4]
{
    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xBrel}

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax]
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax]
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax]
        \pgfmathsetmacro{\lnyC}{\lnyA+1.1*#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
        
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        \draw[black]   (A)--node[pos=0.9,yshift=1ex,xshift=0.5ex] {\small #4}
                    (B)--
                    (C)-- 
                    cycle;
    }
}

%\newcommand{\drawsquare}[3]{\draw[thick,black,fill=#3] (#1,#2)--(#1,#2+1)--(#1+1,#2+1)--(#1+1,#2)--cycle;}


%\begin{document}
\begin{tikzpicture}
\begin{axis}[ticklabel style={{font=\Large}}, major tick length={2pt}, every tick/.style={{black, line cap=round}}, axis on top, legend style={{draw=none, font=\Large, at={(0.03,0.03)}, anchor=south west,ymin=0,ymax=5,xmin=10^-6,xmax=0.2*10^-2, fill=none, legend cell align=left}}, xmode={log}, legend style={{draw=none, font=\small, at={(0.97,0.97)}, anchor=north east, fill=none, legend cell align=left}}, xlabel={\Large RMSE $\varepsilon$ [/]}, ylabel={\Large Normalised Cost [/] },ylabel near ticks, yticklabel pos=right,legend style={font=\scriptsize},every axis plot/.append style={thick}]


        
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%NON NESTED

%        
        \addplot[mark={*}, mark size={2.5pt}, line cap={round}, mark options={solid}, color={rgb,255:red,255;green,89;blue,77}]
        table[row sep={\\}]
        {
            \\
%            0.0028780652145494676  1392.553488366  \\
%            0.002213896318884206  1392.562828273  \\
%            0.0017029971683724659  1392.571557067  \\
%            0.0013099978218249738  1392.580305745  \\
            0.0010076906321730566    0.9985055082811926 \\
            0.0007751466401331204     0.9903205053019548\\
            0.0005962666462562465    1.3803789261198836 \\
            0.00045866665096634343   2.351531226812442 \\
            0.0003528205007433411    2.5547712083332663 \\
            0.00027140038518718546   3.607280888370777  \\
            0.00020876952706706575    4.358873954687506  \\
            0.00016059194389774287    3.9037844016184637  \\
            0.00012353226453672527    3.1861641282697826 \\
            9.502481887440405e-5       2.1663965530543994 \\
            7.309601451877234e-5       3.089682293887322  \\
            5.6227703475978725e-5      4.430999456856593 \\
            4.3252079596906715e-5      4.576315032627905 \\
            3.3270830459159006e-5      3.9769832664894333  \\
            2.559294650704539e-5        2.894496740390511  \\
        }
        ;
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%GLOBAL NESTED
%
        \addplot[mark={triangle*}, mark size={2.5pt}, line cap={round}, mark options={solid}, color={rgb,255:red,255;green,122;blue,40}]
        table[row sep={\\}]
        {
            \\
%%                        0.0028780652145494676  1432.111537889  \\
%%            0.002213896318884206  1432.1198854689999  \\
%%            0.0017029971683724659  1432.162074638  \\
%%            0.0013099978218249738  1432.170760256  \\
            0.0010076906321730566   1.026892104647306  \\
            0.0007751466401331204    0.9461075233026821   \\
            0.0005962666462562465    0.9497648569949858   \\
            0.00045866665096634343   0.9497642476603236   \\
            0.0003528205007433411    0.9518702857244368  \\
            0.00027140038518718546   1.083079479594882  \\
            0.00020876952706706575   1.2568133964674828   \\
            0.00016059194389774287   1.2425842156960027   \\
            0.00012353226453672527   1.4697607883034112    \\
            9.502481887440405e-5     2.0680374446303063    \\
            7.309601451877234e-5     2.035263059383444    \\
            5.6227703475978725e-5    1.3644777280773275    \\
            4.3252079596906715e-5    1.851191156580988    \\
            3.3270830459159006e-5    1.5720902316162064    \\
            2.559294650704539e-5     1.2626855799557613     \\
            1.9686881928496454e-5    1.6076177631731712   \\
            1.5143755329612655e-5    1.5541267894723327    \\
            1.1649042561240503e-5    1.8573630192932136    \\
            8.960801970185002e-6     1.533087940390702    \\
            6.892924592450002e-6     1.169142205176651     \\
        }
        ;
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%LOCAL NESTED




        \addplot[mark={star}, mark size={2.5pt}, line cap={round}, mark options={solid}, color={rgb,255:red,0;green,179;blue,89}]
        table[row sep={\\}]
        {
            \\
%            0.0028780652145494676  1394.635561854  \\
%            0.002213896318884206  1394.6457996079998  \\
%            0.0017029971683724659  1394.655382903  \\
%            0.0013099978218249738  1394.664975403  \\
            0.0010076906321730566   1.  \\
            0.0007751466401331204   1.  \\
            0.0005962666462562465   1.  \\
            0.00045866665096634343  1.  \\
            0.0003528205007433411   1.  \\
            0.00027140038518718546  1.  \\
            0.00020876952706706575  1.  \\
            0.00016059194389774287  1.  \\
            0.00012353226453672527  1.  \\
            9.502481887440405e-5    1.  \\
            7.309601451877234e-5    1.  \\
            5.6227703475978725e-5   1.  \\
            4.3252079596906715e-5   1.  \\
            3.3270830459159006e-5   1.  \\
            2.559294650704539e-5    1.  \\
            1.9686881928496454e-5   1.  \\
            1.5143755329612655e-5   1.  \\
            1.1649042561240503e-5   1.  \\
            8.960801970185002e-6    1. \\
            6.892924592450002e-6    1.  \\
            5.302249686500001e-6    1.  \\
        }
        ;
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5         





 %  \littletriangle{0.15}{0.1}{0.45}{2};
  %  \littletriangle{0.15}{0.1}{0.27}{1};
\end{axis}
\node at (3.5,6.5) {\Large ---Relative Runtime---};

\end{tikzpicture}
%\end{document}


==> level6.tex <==

\begin{tikzpicture}

    \node at (3.5,6.5) {\large ----------- Level 6 ------------};

\end{tikzpicture}


==> level7.tex <==

\begin{tikzpicture}

    \node at (3.5,6.5) {\large ----------- Level 7 ------------};

\end{tikzpicture}


==> level77.tex <==

\begin{tikzpicture}

    \node at (3.5,6.5) {\large ------ Level 7 ------};

\end{tikzpicture}


==> level8.tex <==

\begin{tikzpicture}

    \node at (3.5,6.5) {\large ----------- Level 8 ------------};

\end{tikzpicture}


==> level88.tex <==

\begin{tikzpicture}

    \node at (3.5,6.5) {\large ------- Level 8 -------};

\end{tikzpicture}

